Bi-level Contrastive Learning for Knowledge-Enhanced Molecule Representations

Molecular representation learning is vital for various downstream applications, including the analysis and prediction of molecular properties and side effects. While Graph Neural Networks (GNNs) have been a popular framework for modeling molecular data, they often struggle to capture the full complexity of molecular representations. In this paper, we introduce a novel method called GODE, which accounts for the dual-level structure inherent in molecules. Molecules possess an intrinsic graph structure and simultaneously function as nodes within a broader molecular knowledge graph. GODE integrates individual molecular graph representations with multi-domain biochemical data from knowledge graphs. By pre-training two GNNs on different graph structures and employing contrastive learning, GODE effectively fuses molecular structures with their corresponding knowledge graph substructures. This fusion yields a more robust and informative representation, enhancing molecular property predictions by leveraging both chemical and biological information. When fine-tuned across 11 chemical property tasks, our model significantly outperforms existing benchmarks, achieving an average ROC-AUC improvement of 12.7% for classification tasks and an average RMSE/MAE improvement of 34.4% for regression tasks. Notably, GODE surpasses the current leading model in property prediction, with advancements of 2.2% in classification and 7.2% in regression tasks.

==> figures/ablation_study.tex <==
\begin{figure*}[!h]
    \begin{minipage}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{figures/ablation_config.pdf}
        \includegraphics[width=\linewidth]{figures/ablation_heatmap.pdf}
        \centering
        \parbox{0.9\linewidth}{
            \caption{\textbf{Ablation Study of \textsc{Gode}.} ``Pret.'': K-GNN pre-training. ``Cont'': contrastive learning. ``Embedding'': input to MLP for fine-tuning. The best setting is \colorbox{blue!8}{\makebox(18,5){shaded}}. The best result for each task is \textbf{\textcolor{yellow}{highlighted}}.}
            \label{fig:ablation_study}
        }
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{figures/kg_size_perf.pdf}
        \parbox{0.8\linewidth}{
            \centering
            \caption{\textbf{Performance by the sizes of KG}.}
            \label{fig:kg_size_perf}
        }
        \includegraphics[width=0.9\linewidth]{figures/kgnn_pretraining.pdf}
        \centering
        \parbox{0.8\linewidth}{
            \caption{\textbf{Performance of KG-level (K-GNN) pre-training tasks by time.} We report the means and standard deviation based on five runs with different random seeds.}
            \label{fig:kgnn_pretrain}
        }
    \end{minipage}
    \vspace{-1em}
\end{figure*}


==> figures/kg_size_perf.tex <==
\begin{figure}[!t]
  \centering
  \vspace{-0.5em}
  \includegraphics[width=\linewidth]{figures/kg_size_perf.pdf}
  \vspace{-2em}
\caption{\textbf{Performance by the sizes of KG}.}
\label{fig:kg_size_perf}
  \vspace{-1.5em}
\end{figure}


==> tables/ablation_cls.tex <==
\begin{table*}[!t]
\centering
\caption{\textbf{Ablation study of \textsc{Gode} on classification tasks.} Top-3 and top-1 results are highlighted in \textbf{bold} and \textcolor{red}{\textbf{red}}, respectively. The best setting is shaded.}

\resizebox{\textwidth}{!}{

\begin{tabular}{ccccccccccccc}
\toprule
&\multicolumn{5}{c}{\textbf{Variants}} & \textbf{BBBP} & \textbf{SIDER} & \textbf{ClinTox} & \textbf{BACE} & \textbf{Tox21} & \textbf{ToxCast} \\

\midrule

\textbf{Case} &\textbf{KGE} &\textbf{$\kappa$-hop} &\textbf{Pret.} &\textbf{Cont.} &\textbf{Embedding}\\
\circled{1} &\cmark & \xmark &\xmark &\xmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KGE}}$
& $89.2 \pm 2.2$
& $62.7 \pm 2.1$
& $89.5 \pm 3.5$
& $81.7 \pm 1.6$
& $77.4 \pm 2.9$
& $62.4 \pm 1.7$
\\
\circled{2} &\xmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $92.6 \pm 1.5$
& $\textbf{64.8} \pm \textbf{0.6}$
& $90.2 \pm 1.9$
& $\textbf{84.3} \pm \textbf{1.7}$
& $77.8 \pm 2.3$
& $66.8 \pm 2.3$

\\

\circled{3} &\cmark &$\kappa=2$ &\cmark &\xmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textcolor{red}{\textbf{93.5} \pm \textbf{1.3}}$
& $63.1 \pm 1.5$
& $\textbf{90.6} \pm \textbf{2.1}$
& $83.7 \pm 2.5$
& $\textbf{81.4} \pm \textbf{2.3}$
& $68.0 \pm 1.4$

\\

\rowcolor{blue!8}\circled{4} &\cmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textbf{93.4} \pm \textbf{1.0}$
& $\textcolor{red}{\textbf{64.9} \pm \textbf{1.3}}$
& $\textcolor{red}{\textbf{91.5} \pm \textbf{1.4}}$
& $\textbf{85.8} \pm \textbf{1.6}$
& $\textcolor{red}{\textbf{83.8} \pm \textbf{1.9}}$
& $\textbf{69.2} \pm \textbf{1.1}$

\\




\circled{5} &\cmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}}$
& $92.9 \pm 0.9$
& $\textbf{63.3} \pm \textbf{1.1}$
& $\textcolor{red}{\textbf{91.5} \pm \textbf{2.2}}$
& $83.2 \pm 1.1$
& $78.7 \pm 2.0$
& $\textcolor{red}{\textbf{69.6} \pm \textbf{1.9}}$
\\

\circled{6} &\cmark &$\kappa=3$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textbf{93.1} \pm \textbf{1.1}$
& $61.5 \pm 2.3$
& $90.1 \pm 1.2$
& $\textcolor{red}{\textbf{85.9} \pm \textbf{1.8}}$
& $\textbf{80.3} \pm \textbf{1.9}$
& $68.8 \pm 4.1$


\\
\circled{7} &\cmark &$\kappa=3$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}}$
& $92.5 \pm 1.9$
& $62.8 \pm 0.7$
& $90.3 \pm 1.9$
& $82.4 \pm 3.1$
& $77.9 \pm 0.6$
& $\textbf{69.0} \pm \textbf{2.7}$
\\

\bottomrule
\end{tabular}
}
\label{tab:ablation_study_cls}
\end{table*}

==> tables/ablation_rgr.tex <==
\begin{table*}[!t]
\centering
\caption{\textbf{Ablation study of \textsc{Gode} on regression tasks.} Top-3 and top-1 results are highlighted in \textbf{bold} and \textcolor{red}{\textbf{red}}, respectively. The best setting is shaded.}

\resizebox{\textwidth}{!}{

\begin{tabular}{cccccccccccc}
\toprule
&\multicolumn{5}{c}{\textbf{Variants}} & \textbf{FreeSolv} & \textbf{ESOL} & \textbf{Lipophilicity} & \textbf{QM7} & \textbf{QM8} \\
\midrule
\textbf{Case} &\textbf{KGE} &\textbf{$\kappa$-hop} &\textbf{Pret.} &\textbf{Cont.} &\textbf{Embedding}\\
\circled{1} &\cmark & \xmark &\xmark &\xmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KGE}}$
& $2.341 \pm 0.382$
& $1.205 \pm 0.114$
& $0.829 \pm 0.049$
& $119.9 \pm 2.1$
& $0.032 \pm 0.003$
\\
\circled{2} &\xmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textbf{1.664} \pm \textbf{0.420}$
& $\textbf{0.912} \pm \textbf{0.061}$
& $\textbf{0.731} \pm \textbf{0.086}$
& $102.9 \pm 1.9$
& $\textbf{0.025} \pm \textbf{0.003}$

\\

\circled{3} &\cmark &$\kappa=2$ &\cmark &\xmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $1.995 \pm 0.223$
& $\textbf{0.998} \pm \textbf{0.021}$
& $0.755 \pm 0.093$
& $\textbf{80.1}  \pm \textbf{1.2}$
& $0.028 \pm 0.002$
\\


\rowcolor{blue!8}\circled{4} &\cmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textcolor{red}{\textbf{1.495} \pm \textbf{0.343}}$
& $\textcolor{red}{\textbf{0.910} \pm \textbf{0.028}}$
& $\textcolor{red}{\textbf{0.723} \pm \textbf{0.052}}$
& $\textcolor{red}{\textbf{73.0}  \pm \textbf{3.8}}$
& $\textcolor{red}{\textbf{0.021} \pm \textbf{0.001}}$

\\

\circled{5} &\cmark &$\kappa=2$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}}$
& $1.877 \pm 0.228$
& $1.012 \pm 0.085$
& $\textcolor{red}{\textbf{0.723} \pm \textbf{0.069}}$
& $92.3 \pm 2.9$
& $0.028 \pm 0.002$

\\
\circled{6} &\cmark &$\kappa=3$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}} \oplus \mathbf{h}_{\textrm{KG}}$
& $\textbf{1.744} \pm \textbf{0.415}$
& $1.134 \pm 0.112$
& $0.770 \pm 0.061$
& $\textbf{77.0}  \pm \textbf{4.9}$
& $\textbf{0.024} \pm \textbf{0.004}$
\\
\circled{7} &\cmark &$\kappa=3$ &\cmark &\cmark &$\mathbf{h}_{\textrm
{MG}}$
& $1.779 \pm 0.191$
& $1.007 \pm 0.226$
& $\textbf{0.758} \pm \textbf{0.029}$
& $85.4  \pm 3.3$
& $0.030 \pm 0.001$
\\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\label{tab:ablation_study_rgr}
\end{table*}

==> tables/add_ablation.tex <==
\begin{table*}[h]
\centering
\caption{\textbf{Study the effect of bi-level self-supervised pre-training.} Contrastive learning is conducted between M-GNN and K-GNN no matter they are pre-trained or not. Node embedding in K-GNN are initialized by TransE. All predictions are based on the embedding $\mathbf{h}_{\text{MG}} \oplus \mathbf{h}_{\text{f}} \oplus \mathbf{h}_{\text{KG}}$. ``M'' and ``K'' denote M-GNN pre-training and K-GNN pre-training, respectively. $\Delta$ denotes performance gain from \textsc{Gode} \{M:1, K:1\}.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
\multicolumn{14}{c}{\textbf{Classification Tasks} (higher is better)}\\
\toprule
M &K &BBBP &$\Delta$ &SIDER &$\Delta$ &ClinTox &$\Delta$ &BACE &$\Delta$ &Tox21 &$\Delta$ &ToxCast &$\Delta$\\
\midrule
1 &1 & \textbf{94.5} &- &\textbf{67.2} &- & \textbf{94.1} &- &\textbf{91.8} &- &\textbf{84.3} &- &\textbf{73.0} &-
\\
0 &1 
& 92.2 &$\downarrow$ 2.3
& 62.6 &$\downarrow$ 4.6
& 89.4 &$\downarrow$ 4.7
& 89.8 &$\downarrow$ 2.0
& 80.6 &$\downarrow$ 3.7
& 70.8 &$\downarrow$ 2.2
\\
1 &0
& 93.2 &$\downarrow$ 1.3
& 66.7 &$\downarrow$ 0.5
& 90.7 &$\downarrow$ 3.4
& 81.6 &$\downarrow$ 10.2
& 83.1 &$\downarrow$ 1.2
& 71.9 &$\downarrow$ 1.1
\\
0 &0
& 88.9 &$\downarrow$ 5.6
& 62.1 &$\downarrow$ 5.1
& 88.4 &$\downarrow$ 5.7
& 84.1 &$\downarrow$ 7.7
& 81.6 &$\downarrow$ 2.7
& 69.4 &$\downarrow$ 3.6 
\\
\midrule
\\
\multicolumn{14}{c}{\textbf{Regression Tasks} (lower is better)}\\
\toprule
M &K &FreeSolv &$\Delta$ &ESOL &$\Delta$ &Lipo &$\Delta$ &QM7 &$\Delta$ &QM8 &$\Delta$ \\
\midrule
1 &1& \textbf{1.129} &- & \textbf{0.785} &- & 0.743 &- & \textbf{57.2} &- &\textbf{0.014} &-
\\
0 &1
& 1.313 & $\uparrow$ 0.184
& 0.834 & $\uparrow$ 0.049
& \textbf{0.708} & $\downarrow$ 0.035
& 64.6  & $\uparrow$ 7.4
& 0.016 & $\uparrow$ 0.002
\\
1 &0
& 1.563 & $\uparrow$ 0.434
& 0.841 & $\uparrow$ 0.056
& 0.876 & $\uparrow$ 0.133
& 74.4  & $\uparrow$ 17.2
& 0.017 & $\uparrow$ 0.003
\\
0 &0
& 1.944 &$\uparrow$ 0.815
& 0.978 &$\uparrow$ 0.193
& 0.845 &$\uparrow$ 0.102
& 77.9  &$\uparrow$ 20.7
& 0.017 &$\uparrow$ 0.003
\\
\bottomrule

\end{tabular}
}
\label{tb:effects_ssp}
\end{table*}


==> tables/classification.tex <==
\begin{table*}[!h]
\centering
\caption{\textbf{ROC-AUC performance on six \textit{classification} benchmarks (\textit{higher is better}).} We report the mean and standard deviation. Top-3 and top-1 results are highlighted in \textbf{bold} and \textcolor{red}{\textbf{bold red}}, respectively. We highlight the \colorbox{gray!20}{\makebox(64,5){backbone model}}, and the \colorbox{yellow!10}{\makebox(120,5){models that apply the backbone}.} Table split: Non-KG and KG-based methods.
}

\resizebox{0.9\textwidth}{!}{

\begin{tabular}{lrrrrrr}
\toprule
\textbf{Dataset} & \textbf{BBBP} & \textbf{SIDER} & \textbf{ClinTox} & \textbf{BACE} & \textbf{Tox21} & \textbf{ToxCast} \\
\# Molecules   & 2039  & 1427  &1478    &1513  &7831   &8575 \\
\# Tasks       &1      &27     &2       &1     &12     &617\\
\midrule\midrule
GCN~\citep{kipf2016semi}     
& $71.8 \pm 0.9$ 
& $53.6 \pm 0.3$ 
& $62.5 \pm 2.8$ 
& $71.6 \pm 2.0$ 
& $70.9 \pm 0.3$
& $65.0 \pm 6.1$ 
\\
GIN~\citep{xu2018powerful}               
& $65.8 \pm 4.5$ 
& $57.3 \pm 1.6$ 
& $58.0 \pm 4.4$ 
& $70.1 \pm 5.4$ 
& $74.0 \pm 0.8$ 
& $66.7 \pm 1.5$ 
\\
% Weave~\citep{kearnes2016molecular}       
% & $83.7 \pm 6.5$
% & $54.3 \pm 3.4$
% & $82.3 \pm 2.3$ 
% & $79.1 \pm 0.8$ 
% & $74.1 \pm 4.4$ 
% & $67.8 \pm 2.4$ 
% \\
SchNet~\citep{schutt2017schnet}           
& $84.8 \pm 2.2$ 
& $54.5 \pm 3.8$ 
& $71.7 \pm 4.2$ 
& $76.6 \pm 1.1$
& $76.6 \pm 2.5$ 
& $67.9 \pm 2.1$  
\\
MPNN~\citep{gilmer2017neural}         
& $91.3 \pm 4.1$
& $59.5 \pm 3.0$
& $87.9 \pm 5.4$ 
& $81.5 \pm 4.4$ 
& $80.8 \pm 2.4$
& $69.1 \pm 1.3$
\\
DMPNN~\citep{yang2019analyzing}         
& $91.9 \pm 3.0$ 
& $63.2 \pm 2.3$
& $89.7 \pm 4.0$ 
& $85.2 \pm 5.3$
& $\textbf{82.6} \pm \textbf{2.3}$
& $71.8 \pm 1.1$ 
\\
MGCN~\citep{lu2019molecular}            
& $85.0 \pm 6.4$ 
& $55.2 \pm 1.8$ 
& $63.4 \pm 4.2$ 
& $73.4 \pm 3.0$
& $70.7 \pm 1.6$ 
& $66.3 \pm 0.9$
\\
N-GRAM~\citep{liu2019n}                 
& $91.2 \pm 1.3$ 
& $63.2 \pm 0.5$
& $85.5 \pm 3.7$ 
& $87.6 \pm 3.5$
& $76.9 \pm 2.7$ 
& -  
\\
HU. et.al~\citep{hu2019strategies}        
& $70.8 \pm 1.5$
& $62.7 \pm 0.8$
& $72.6 \pm 1.5$ 
& $84.5 \pm 0.7$
& $78.7 \pm 0.4$ 
& $65.7 \pm 0.6$ 
\\
\rowcolor{gray!20} $\textrm{GROVER}_{\textrm{Large, GTrans}}$~\citep{rong2020selfsupervised}     
& $86.2 \pm 3.9$
& $57.6 \pm 1.6$
& $74.7 \pm 4.4$
& $82.5 \pm 4.4$
& $76.9 \pm 2.3$
& $66.7 \pm 2.6$
\\
MGSSL~\citep{zhang2021motifbased}           
& $70.5 \pm 1.1$
& $64.1 \pm 0.7$
& $80.7 \pm 2.1$
& $79.7 \pm 0.8$
& $76.4 \pm 0.4$
& $64.1 \pm 0.7$
\\
MolCLR~\citep{wang2102molclr}
& $73.3 \pm 1.0$
& $61.2 \pm 3.6$
& $89.8 \pm 2.7$
& $82.8 \pm 0.7$
& $74.1 \pm 5.3$
& $65.9 \pm 2.1$
\\
\rowcolor{yellow!10} $\text{MolCLR}_{\text{GTrans}}$~\citep{wang2102molclr}
& $76.7 \pm 2.2$
& $63.3 \pm 2.5$
& $89.3 \pm 3.1$
& $87.7 \pm 1.8$
& $80.2 \pm 3.2$
& $70.4 \pm 2.1$
\\
\midrule
\rowcolor{yellow!10} KGE\_NFM~\citep{ye2021unified} w/ our MolKG
& $92.4 \pm 2.4$
& $\textbf{65.3} \pm \textbf{1.4}$
& $87.3 \pm 2.0$ 
& $78.1 \pm 2.1$
& $79.8 \pm 3.3$ 
& $\textbf{72.6} \pm \textbf{1.8}$ 
\\
$\text{KANO}_{\text{CMPNN}}$~\citep{fang2022geometry}
& $\textbf{92.6} \pm \textbf{1.8}$
& $\textbf{65.5} \pm \textbf{1.6}$
& $\textbf{92.9} \pm \textbf{1.1}$
& $\textbf{90.7} \pm \textbf{3.1}$
& $81.8 \pm 1.1$
& $\textbf{72.5} \pm \textbf{1.9}$
\\
\rowcolor{yellow!10} $\text{KANO}_{\text{GTrans}}$~\citep{fang2023knowledge}
& $\textbf{93.7} \pm \textbf{2.3}$
& $63.8 \pm 1.2$
& $\textbf{93.6} \pm \textbf{0.7}$
& $\textbf{90.4} \pm \textbf{1.5}$
& $\textbf{81.2} \pm \textbf{1.8}$
& $\textbf{72.5} \pm \textbf{1.5}$
\\
\rowcolor{yellow!10} \textsc{Gode} (ours)
& $\textcolor{red}{\textbf{94.5} \pm \textbf{1.9}}$
& $\textcolor{red}{\textbf{67.2} \pm \textbf{1.4}}$
& $\textcolor{red}{\textbf{94.1} \pm \textbf{2.9}}$
& $\textcolor{red}{\textbf{91.8} \pm \textbf{2.2}}$
& $\textcolor{red}{\textbf{84.3} \pm \textbf{1.2}}$
& $\textcolor{red}{\textbf{73.0} \pm \textbf{0.9}}$

\\

\bottomrule
\end{tabular}
}
\label{tab:cls_results}
\end{table*}

==> tables/classification_backbone.tex <==
\begin{table*}[!tp]
\centering
\caption{\textbf{ROC-AUC performance on six \textit{classification} benchmarks (\textit{higher is better}).} We report the mean and standard deviation. Top-3 and top-1 results are highlighted in \textbf{bold} and \textcolor{red}{\textbf{red}}, respectively. The backbone M-GNNs of \textsc{Gode} are shaded.
}

\resizebox{0.9\textwidth}{!}{

\begin{tabular}{lrrrrrr}
\toprule
\textbf{Dataset} & \textbf{BBBP} & \textbf{SIDER} & \textbf{ClinTox} & \textbf{BACE} & \textbf{Tox21} & \textbf{ToxCast} \\
\# Molecules   & 2039  & 1427  &1478    &1513  &7831   &8575 \\
\# Tasks       &1      &27     &2       &1     &12     &617\\
\midrule\midrule
\textbf{Baselines}
\\
GCN~\citep{kipf2016semi}     
& $71.8 \pm 0.9$ 
& $53.6 \pm 0.3$ 
& $62.5 \pm 2.8$ 
& $71.6 \pm 2.0$ 
& $70.9 \pm 0.3$
& $65.0 \pm 6.1$ 
\\
GIN~\citep{xu2018powerful}               
& $65.8 \pm 4.5$ 
& $57.3 \pm 1.6$ 
& $58.0 \pm 4.4$ 
& $70.1 \pm 5.4$ 
& $74.0 \pm 0.8$ 
& $66.7 \pm 1.5$ 
\\
Weave~\citep{kearnes2016molecular}       
& $83.7 \pm 6.5$
& $54.3 \pm 3.4$
& $82.3 \pm 2.3$ 
& $79.1 \pm 0.8$ 
& $74.1 \pm 4.4$ 
& $67.8 \pm 2.4$ 
\\
SchNet~\citep{schutt2017schnet}           
& $84.8 \pm 2.2$ 
& $54.5 \pm 3.8$ 
& $71.7 \pm 4.2$ 
& $76.6 \pm 1.1$
& $76.6 \pm 2.5$ 
& $67.9 \pm 2.1$  
\\
\rowcolor{gray!20} MPNN~\citep{gilmer2017neural}         
& $91.3 \pm 4.1$
& $59.5 \pm 3.0$
& $87.9 \pm 5.4$ 
& $81.5 \pm 4.4$ 
& $80.8 \pm 2.4$
& $69.1 \pm 1.3$
\\
\rowcolor{gray!20} DMPNN~\citep{yang2019analyzing}         
& $91.9 \pm 3.0$ 
& $63.2 \pm 2.3$
& $89.7 \pm 4.0$ 
& $85.2 \pm 5.3$
& $82.6 \pm 2.3$
& $71.8 \pm 1.1$ 
\\
MGCN~\citep{lu2019molecular}            
& $85.0 \pm 6.4$ 
& $55.2 \pm 1.8$ 
& $63.4 \pm 4.2$ 
& $73.4 \pm 3.0$
& $70.7 \pm 1.6$ 
& $66.3 \pm 0.9$
\\
MGSSL~\citep{zhang2021motifbased}           
& $70.5 \pm 1.1$
& $64.1 \pm 0.7$
& $80.7 \pm 2.1$
& $79.7 \pm 0.8$
& $76.4 \pm 0.4$
& $64.1 \pm 0.7$
\\
N-GRAM~\citep{liu2019n}                 
& $91.2 \pm 1.3$ 
& $63.2 \pm 0.5$
& $85.5 \pm 3.7$ 
& $87.6 \pm 3.5$
& $76.9 \pm 2.7$ 
& -  
\\
HU. et.al~\citep{hu2019strategies}        
& $70.8 \pm 1.5$
& $62.7 \pm 0.8$
& $72.6 \pm 1.5$ 
& $84.5 \pm 0.7$
& $78.7 \pm 0.4$ 
& $65.7 \pm 0.6$ 
\\
\rowcolor{gray!20} $\textrm{GROVER}_{\textrm{Large}}$~\citep{rong2020selfsupervised}     
& $89.0 \pm 1.1$
& $56.0 \pm 1.8$
& $73.7 \pm 4.3$
& $80.1 \pm 2.6$
& $73.9 \pm 0.7$
& $66.6 \pm 2.4$
\\
MolCLR~\citep{wang2102molclr}
& $73.3 \pm 1.0$
& $61.2 \pm 3.6$
& $89.8 \pm 2.7$
& $82.8 \pm 0.7$
& $74.1 \pm 5.3$
& $65.9 \pm 2.1$
\\
KANO~\citep{fang2023knowledge}
& $94.7 \pm 2.1$
& $63.8 \pm 1.2$
& $93.6 \pm 0.8$
& $90.4 \pm 1.5$
& $81.2 \pm 1.8$
& $72.1 \pm 1.8$
\\
\midrule
\textbf{\textsc{Gode}} (our method)
\\
w/ MPNN
& $93.8 \pm 3.2$
& $64.4 \pm 3.1$
& $92.1 \pm 4.3$
& $87.8 \pm 2.9$
& $82.3 \pm 3.0$
& $71.5 \pm 1.3$
\\
w/ DMPNN
& $95.3 \pm 1.8$
& $65.3 \pm 3.1$
& $90.2 \pm 2.3$
& $89.2 \pm 3.8$
& $83.3 \pm 1.5$
& $72.6 \pm 0.9$

\\
w/ GROVER
& $93.4 \pm 1.0$
& $64.9 \pm 1.3$
& $91.5 \pm 1.4$
& $85.8 \pm 1.6$
& $83.8 \pm 1.9$
& $69.2 \pm 1.1$
\\
\bottomrule
\end{tabular}
}
\label{tab:cls_results}
\end{table*}

==> tables/finetune_datasets.tex <==
\begin{table}[ht]
\centering
\begin{tabularx}{\textwidth}{|l|X|}
\hline
\textbf{Dataset} & \textbf{Description} \\
\hline
\hline
\textbf{BBBP}~\cite{martins2012bayesian} & Focused on the permeability property of compounds detailing whether a compound can penetrate the blood-brain barrier. \\
\hline
\textbf{SIDER}~\cite{kuhn2016sider} & Chronicles marketed drugs and associates them with potential adverse drug reactions. \\
\hline
\textbf{ClinTox}~\cite{gayvert2016data} & Contrasts FDA-approved drugs against those dismissed due to toxicity concerns during clinical trials. \\
\hline
\textbf{BACE}~\cite{subramanian2016computational} & Collection around compounds potential as inhibitors of human β-secretase 1 (BACE-1). \\
\hline
\textbf{Tox21}~\cite{tox21} & Public database offering insights into the toxicity of compounds, utilized in the 2014 Tox21 Data Challenge. \\
\hline
\textbf{ToxCast}~\cite{richard2016toxcast} & Contains multiple toxicity labels derived from high-throughput screening tests for thousands of compounds. \\
\hline
\textbf{QM7}~\cite{blum2009970} & Subset of GDB-13 documenting computed atomization energies of stable, synthetically achievable organic molecules. \\
\hline
\textbf{QM8}~\cite{ramakrishnan2015electronic} & Houses computer-generated quantum mechanical attributes, including electronic spectra and excited state energy of small molecules. \\
\hline
\textbf{ESOL}~\cite{delaney2004esol} & Chronicles the solubility attributes of different compounds. \\
\hline
\textbf{Lipophilicity}~\cite{gaulton2012chembl} & From ChEMBL database, detailing lipophilicity derived from octanol/water distribution coefficient experiments. \\
\hline
\textbf{FreeSolv}~\cite{mobley2014freesolv} & From Free Solvation Database, it enumerates hydration free energy of molecules in water, both from experimental data and alchemical free energy calculations. \\
\hline
\end{tabularx}
\caption{Overview of Molecular Property Prediction Datasets}
\end{table}


==> tables/regression.tex <==
\begin{table*}[!h]
\centering
\caption{\textbf{RMSE (for FreeSolv, ESOL, Lipophilicity) and MAE (for QM7/8) performance on five \textit{regression} benchmarks (\textit{lower is better}).} Top-3 and top-1 results are highlighted in \textbf{bold} and \textcolor{red}{\textbf{bold red}}, respectively. We highlight the \colorbox{gray!20}{\makebox(64,5){backbone model}}, and the \colorbox{yellow!10}{\makebox(120,5){models that apply the backbone}}.
}
\label{tab:rgr_results}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lrrrrr}
\toprule
\textbf{Datasets} & \textbf{FreeSolv} & \textbf{ESOL} & \textbf{Lipophilicity} & \textbf{QM7} & \textbf{QM8} \\
\# Molecules   & 642    & 1128   & 4200    & 6830      & 21786             \\
\# Tasks       & 1      & 1      & 1       & 1         & 12                \\
\midrule\midrule
GCN~\citep{kipf2016semi}                 
& $2.870 \pm 0.140$
& $1.430 \pm 0.050$
& $0.712 \pm 0.049$
& $122.9 \pm 2.2$
& $0.037 \pm 0.001$ 
\\
GIN~\citep{xu2018powerful}       
& $2.765 \pm 0.180$
& $1.452 \pm 0.020$
& $0.850 \pm 0.071$ 
& $124.8 \pm 0.7$ 
& $0.037 \pm 0.001$
\\
% Weave~\citep{kearnes2016molecular} 
% & $2.398 \pm 0.250$ 
% & $1.158 \pm 0.055$
% & $0.813 \pm 0.042$
% & $94.7  \pm 2.7$  
% & $0.022 \pm 0.001$ 
% \\
SchNet~\citep{schutt2017schnet}  
& $3.215 \pm 0.755$ 
& $1.045 \pm 0.064$ 
& $0.909 \pm 0.098$ 
& $74.2  \pm 6.0$  
& $0.020 \pm 0.002$ 
\\
MPNN~\citep{gilmer2017neural}            
& $1.621 \pm 0.952$ 
& $1.167 \pm 0.430$ 
& $\textbf{0.672} \pm \textbf{0.051}$
& $111.4 \pm 0.9$
& $\textbf{0.015} \pm \textbf{0.001}$
\\
DMPNN~\citep{yang2019analyzing}            
& $1.673 \pm 0.082$ 
& $1.050 \pm 0.008$ 
& $0.683 \pm 0.016$ 
& $103.5 \pm 8.6$ 
& $\textbf{0.016} \pm \textbf{0.001}$
\\
MGCN~\citep{lu2019molecular}            
& $3.349 \pm 0.097$ 
& $1.266 \pm 0.147$ 
& $1.113 \pm 0.041$ 
& $77.6  \pm 4.7$
& $0.022 \pm 0.002$
\\
N-GRAM~\citep{liu2019n}                  
& $2.512 \pm 0.190$ 
& $1.100 \pm 0.160$
& $0.876 \pm 0.033$ 
& $125.6 \pm 1.5$
& $0.032 \pm0.003$
\\
HU. et.al~\citep{hu2019strategies}           
& $2.764 \pm 0.002$
& $1.100 \pm 0.006$
& $0.739 \pm 0.003$
& $113.2 \pm 0.6$
& $0.022 \pm 0.001$
\\
\rowcolor{gray!20} $\textrm{GROVER}_{\textrm{Large, GTrans}}$~\citep{rong2020selfsupervised}    
& $2.445 \pm 0.761$
& $1.028 \pm 0.145$
& $0.890 \pm 0.050$
& $95.3 \pm 5.6$
& $0.020 \pm 0.003$
\\
MolCLR~\citep{wang2102molclr} 
& $2.301 \pm 0.247$
& $1.113 \pm 0.023$
& $0.789 \pm 0.009$
& $90.0  \pm 1.7$
& $0.019 \pm 0.013$
\\
\rowcolor{yellow!10} $\text{MolCLR}_{\text{GTrans}}$~\citep{wang2102molclr}
& $2.124 \pm 0.223$
& $0.982 \pm 0.109$
& $0.767 \pm 0.064$
& $88.9 \pm 4.8$
& $0.018 \pm 0.002$
\\
\midrule
\rowcolor{yellow!10} KGE\_NFM~\citep{ye2021unified} w/ our MolKG      
& $1.942 \pm 0.441$
& $1.027 \pm 0.201$
& $0.877 \pm 0.071$ 
& $87.6 \pm 3.2$
& $\textbf{0.016} \pm \textbf{0.001}$ 
\\
$\text{KANO}_{\text{CMPNN}}$~\citep{fang2022geometry}
& $\textbf{1.320} \pm \textbf{0.244}$
& $\textbf{0.902} \pm \textbf{0.104}$
& $\textcolor{red}{\textbf{0.641} \pm \textbf{0.012}}$
& $\textbf{66.5} \pm \textbf{3.7}$
& $\textcolor{red}{\textbf{0.014} \pm \textbf{0.001}}$
\\
\rowcolor{yellow!10} $\text{KANO}_{\text{GTrans}}$~\citep{fang2023knowledge} 
& $\textbf{1.443} \pm \textbf{0.315}$
& $\textbf{0.914} \pm \textbf{0.092}$
& $\textbf{0.651} \pm \textbf{0.018}$
& $\textbf{63.6}  \pm \textbf{4.1}$
& $\textcolor{red}{\textbf{0.014} \pm \textbf{0.002}}$
\\
\rowcolor{yellow!10} \textsc{Gode} (ours)
& $\textcolor{red}{\textbf{1.129} \pm \textbf{0.314}}$
& $\textcolor{red}{\textbf{0.785} \pm \textbf{0.128}}$
& $0.743 \pm 0.043$
& $\textcolor{red}{\textbf{57.2}  \pm \textbf{3.0}}$
& $\textcolor{red}{\textbf{0.014} \pm \textbf{0.001}}$

\\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/rel_removal.tex <==
\begin{table*}[t]
\centering
\caption{Effect of Relationship Exclusion on Model Performance.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Knowledge Graph} & \textbf{BBBP} &\textbf{SIDER} &\textbf{ClinTox} & \textbf{BACE} &\textbf{Tox21} &\textbf{ToxCast} \\ \midrule
MolKG & 94.5 &67.2 &94.1 & 91.8 & 84.3 & 73.0\\
w/o \textit{indication} & 93.8 (\textdownarrow 0.7) &65.7 (\textdownarrow 1.5) & 93.4 (\textdownarrow 0.7) & 91.6 (\textdownarrow 0.2) & 84.2 (\textdownarrow 0.1) & 73.0 (--0.0) \\
w/o \textit{xlogp3} \& \textit{xlogp3-aa} & 93.7 (\textdownarrow 0.8) &66.0 (\textdownarrow 1.2) & 94.2 (\textuparrow 0.1) & 91.1 (\textdownarrow 0.7) & 83.0 (\textdownarrow 1.3) & 72.8 (\textdownarrow 0.2) \\
w/o \textit{tautomer\_cnt} \& \textit{covalent\_unit\_cnt} & 94.3 (\textdownarrow 0.2) &66.5 (\textdownarrow 0.7) &92.9 (\textdownarrow 1.2) & 90.9 (\textdownarrow 0.9) & 83.5 (\textdownarrow 0.8) & 72.5 (\textdownarrow 0.5) \\
w/o \textit{nbr\_2d} \& \textit{nbr\_3d} \& \textit{has\_same\_conn} & 94.9 (\textuparrow 0.4) &67.5 (\textuparrow 0.3) &93.6 (\textdownarrow 0.5) & 91.3 (\textdownarrow 0.5) & 84.3 (--0.0) & 72.7 (\textdownarrow 0.3) \\ \bottomrule
\end{tabular}}
\label{tb:rel_removal}
\end{table*}

